Five-brane webs, Higgs branches and unitary/orthosymplectic magnetic quivers

We study the Higgs branch of 5d superconformal theories engineered from brane webs with orientifold five-planes. We propose a generalization of the rules to derive magnetic quivers from brane webs pioneered in arXiv:2004.04082, by analyzing theories that can be described with a brane web with and without O5 planes. Our proposed magnetic quivers include novel features, such as hypermultiplets transforming in the fundamental-fundamental representation of two gauge nodes, antisymmetric matter, and $\mathbb{Z}_2$ gauge nodes. We test our results by computing the Coulomb and Higgs branch Hilbert series of the magnetic quivers obtained from the two distinct constructions and find agreement in all cases.

==> CBHilbertSeries.tex <==
\section{Coulomb branch Hilbert series of magnetic quivers}\label{secCBHS}
In this section, we will present the Hilbert series of the Coulomb branch of the magnetic quivers obtained in earlier sections. We will use the \emph{monopole formula} prescribed in \cite{Cremonesi:2013lqa} which essentially counts the number of \emph{dressed} monopole operators according to their conformal dimension. We refer the readers to Appendix \ref{app1} for a brief description of the monopole formula and using it to compute the Hilbert series. Since we are computing the Hilbert series as a non-trivial check to support the equivalence of Coulomb branches of the proposed unitary and orthosymplectic magnetic quivers, it suffices to see the matching of the Hilbert series up to certain orders of $t$ (the counting parameter) to see the explicit matching. Of course, the Hilbert series themselves are interesting objects and it would be worthwhile to explore the refined Hilbert series and to extract the generators of the chiral ring of the moduli spaces of the magnetic quivers obtained in previous sections. We leave this exercise for future work.   
%*********************************************************
%*********************************************************
\subsection{O5$^{-}$ \textemdash \, O5$^{-}$}
%*********************************************************
%*********************************************************
\subsection{O5$^{+}$ \textemdash \, O5$^{+}$}
The unitary and orthosymplectic magnetic quivers for $+_{1,M}$ theory are given in figure \ref{xxU} and figure \ref{xxOS} respectively. For small values of $M$, we have explicitly checked the matching of the Hilbert series which are given below:
\begin{align}
\text{HS}_{M=1} &= \frac{t^{10}+8 t^9+40 t^8+107 t^7+199 t^6+234 t^5+199 t^4+107 t^3+40 t^2+8 t+1}{(1-t)^{10} \, (1+t)^5} \nonumber \\
\text{HS}_{M=2} &= 1+21t+249t^2+2188t^3+15657t^4+95340t^5 + \ldots ~.
\end{align}
For $K_{1,N}^1$ theory, the Hilbert series for unitary case for small values of $N$ are given below:
\begin{align}
\text{HS}_{N=1}^{\text{unitary}} &= \frac{t^4+2t^3+4 t^2+2 t+1}{(1-t)^4 \, (1+t)^2} \nonumber \\
\text{HS}_{N=2}^{\text{unitary}} &= 1+12t+85t^2+450t^3+1954t^4+7232t^5 + \ldots ~.
\end{align}
Unfortunately the orthosympletic quiver in this case is a bad quiver, so we can not compute its Coulomb branch Hilbert series. However, the Higgs branch Hilbert series can be computed and we see the matching.
%*********************************************************
%*********************************************************
\subsection{O5$^{-}$ \textemdash \, O5$^{+}$}
%*********************************************************
%*********************************************************
\subsection{$\widetilde{\text{O5}}^{+}$ \textemdash \, $\widetilde{\text{O5}}^{+}$}
%*********************************************************
%*********************************************************
\subsection{$\widetilde{\text{O5}}^{+}$ \textemdash \, $\widetilde{\text{O5}}^{-}$}
